Exploring the Hyperparameter Landscape of Adversarial Robustness

Adversarial training shows promise as an approach for training models that are robust towards adversarial perturbation. In this paper, we explore some of the practical challenges of adversarial training. We present a sensitivity analysis that illustrates that the effectiveness of adversarial training hinges on the settings of a few salient hyperparameters. We show that the robustness surface that emerges across these salient parameters can be surprisingly complex and that therefore no effective one-size-fits-all parameter settings exist. We then demonstrate that we can use the same salient hyperparameters as tuning knob to navigate the tension that can arise between robustness and accuracy. Based on these findings, we present a practical approach that leverages hyperparameter optimization techniques for tuning adversarial training to maximize robustness while keeping the loss in accuracy within a defined budget.

==> related.tex <==
\section{Related Work}
\label{related}

Related work falls into two areas: adversarial robustness und hyperparameter optimization (HPO). We reviewed the most relevant work on adversarial robustness in Section~\ref{sec:background} and focus on this section on HPO. 

HPO \cite{bergstrahpo2011,bergstrabengiohpo,snoek2012} is the problem of choosing optimal hyper parameter settings for learning algorithms. HPO is commonly applied to tune training parameters such as learning rates and batch sizes. Our work on auto-tuning robustness parameters builds  on prior work in HPO by adapting existing HPO strategies to our problem of tuning adversarial training parameters. Unlike in standard HPO scenarios model accuracy is not the only objective function when tuneing adversarial training; instead there are two objective function: robustness and accuracy and existing HPO techniques need to be adapted to account for the dual objective function setting. 
%So far we have experimented with adapted versions of the Tree-structured Parzen estimator (TPE) ~\cite{bergstrahpo2011} and random search \cite{bergstrabengiohpo} into our RaaS service and are planning to extend the set of supported strategies further in the future. 



